The gem5 Simulator: Version 20.0+

The open-source and community-supported gem5 simulator is one of the most popular tools for computer architecture research. This simulation infrastructure allows researchers to model modern computer hardware at the cycle level, and it has enough fidelity to boot unmodified Linux-based operating systems and run full applications for multiple architectures including x86, Arm, and RISC-V. The gem5 simulator has been under active development over the last nine years since the original gem5 release. In this time, there have been over 7500 commits to the codebase from over 250 unique contributors which have improved the simulator by adding new features, fixing bugs, and increasing the code quality. In this paper, we give and overview of gem5's usage and features, describe the current state of the gem5 simulator, and enumerate the major changes since the initial release of gem5. We also discuss how the gem5 simulator has transitioned to a formal governance model to enable continued improvement and community support for the next 20 years of computer architecture research.

==> changes/arm-fastmodel.tex <==
\subsection[Arm Fastmodel]{Arm Fastmodel\footnote{By Gabriel Black}}

Haven't heard anything back, yet.


==> changes/gem5-and-sst-integration.tex <==

\subsection[gem5 and SST Integration]{gem5 and SST Integration\footnote{by Curtis Dunham}}
\label{sec:sst}

Haven't head back, yet.


==> changes/memory-traces-and-traffic-generator.tex <==
\subsection[Memory Traces and Traffic Generator]{Memory Traces and Traffic Generator\footnote{by Andreas Hanson}}

Haven't heard back, yet.


==> changes/minor-in-order-cpu-model.tex <==
\subsection[The Minor In-Order CPU Model]{The Minor In-Order CPU Model\footnote{by Andrew Bardsley}}

Haven't heard back, yet.


